Fast Laplace transforms on quantum computers

While many classical algorithms rely on Laplace transforms, it has remained an open question whether these operations could be implemented efficiently on quantum computers. In this work, we introduce the Quantum Laplace Transform (QLT), which enables the implementation of $N\times N$ discrete Laplace transforms on quantum states encoded in $\lceil \log_2(N)\rceil$-qubits. In many cases, the associated quantum circuits have a depth that scales with $N$ as $O(\log(\log(N)))$ and a size that scales as $O(\log(N))$, requiring exponentially fewer operations and double-exponentially less computational time than their classical counterparts. These efficient scalings open the possibility of developing a new class of quantum algorithms based on Laplace transforms, with potential applications in physics, engineering, chemistry, machine learning, and finance.

==> boilerplate.tex <==
\DeclareGraphicsRule{.tif}{png}{.png}{`convert #1 `dirname #1`/`basename #1 .tif`.png}
%%%%%Shorthand symbols
\newcommand{\tr}{\operatorname{Tr}}
\newcommand{\ket}[1]{\left | #1 \right \rangle}
\newcommand{\bra}[1]{\left \langle #1 \right |}
\newcommand{\proj}[1]{\ket{#1}\!\!\bra{#1}}
\newcommand{\rem}[1] {\textcolor[gray]{0.7}{#1}}
\newcommand{\todo}[1] {\textcolor{red}{#1}}
\newcommand{\apcha}[1] {\textcolor{blue}{#1}}
\newcommand{\jmcha}[1] {\textcolor{red}{#1}}
\definecolor{col1}{rgb}{.5,.0,.0}  
\definecolor{col2}{rgb}{.2,.5,.2}  
\definecolor{col3}{rgb}{.5,.5,.5}  
%%%%%%

\usepackage[a4paper,inner=3.0cm,outer=3.0cm,top=2.9cm,bottom=3cm,pdftex]{geometry}

\setlength{\parindent}{0cm}
\setlength{\parskip}{.2cm plus 0.05cm minus 0.05cm}

% Define some useful environments:
% Comment
\newenvironment{comment}
{
   \vspace{3mm}\hrule\vspace{3mm}
   \textbf{Comment:} \begin{itshape}\small 
}
{
    \end{itshape}
}

\newenvironment{response}
{\textbf{Response: }}
{}

\newenvironment{suggest}[1]
{
    \textcolor{col1}{\textbf{Suggestion (#1):} }
    \begin{color}{col1}
}
{\end{color}}

\pagestyle{fancy}
\fancyhead{}
\fancyhead[LO,LE]{\color{col3}\sffamily \small Response to Referee comments}
\fancyhead[RO,RE]{\color{col3}\sffamily \small \textit{NCOMMS-24-05781-T}} %Insert paper code/author name here
\renewcommand{\headrulewidth}{0pt}

{\normalsize}

%Quote (it already exists as an environment, want to alter it)
\renewenvironment{quote}{%
  \list{}{%
    \leftmargin0.4cm   % this adjusts the width
    \rightmargin\leftmargin
  }
  \item\relax}
{\endlist \vspace{-1mm}}

